LoopVL: Recurrent Visual Intelligence

We introduce LoopVL to study whether Loop Transformers can be effectively extended to vision- language models. LoopVL combines Module-Loop and Model-Loop computation to iteratively update a unified vision-language state through shared modules. We train LoopVL from scratch through language pre-training, multimodal training, and post-training. LoopVL outperforms a range of similarly sized and larger non-recurrent models on multimodal understanding and visual reasoning benchmarks. We also observe Visual Aha Moments in LoopVL, characterized by pronounced shifts in visual attention across loops. LoopVL provides practical evidence for recurrent vision-language modeling and offers an intuitive perspective on how shared parameters can support deeper multimodal computation over continuously evolving visual-language states.

==> ai2style/defns.tex <==
%
% A useful set of commands
\usepackage{mathtools}
\usepackage{dsfont}
\usepackage[dvipsnames]{xcolor}
\usepackage[colorinlistoftodos]{todonotes}
\usepackage{booktabs}
\usepackage{xfrac}
\usepackage{bbm}

\usepackage{algpseudocode}
\usepackage{algorithm}
\usepackage{algorithmicx}

\usepackage[most]{tcolorbox}
\usepackage{xparse}
\usepackage{lipsum}
\usepackage{changepage}
\usepackage{enumitem}

\newcommand{\qedwhite}{\hfill \ensuremath{\Box}}

%http://www-db.stanford.edu/~manku/latex.html
%The itemize environment can be replaced by:
\newcommand{\squishlist}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}      \setlength{\parsep}{3pt}
      \setlength{\topsep}{3pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishlisttwo}{
   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{0pt}    \setlength{\parsep}{0pt}
      \setlength{\topsep}{0pt}     \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{2em} \setlength{\labelwidth}{1.5em}
      \setlength{\labelsep}{0.5em} } }

\newcommand{\squishend}{
    \end{list}  }

%Example usage: \squishlist    %% \begin{itemize}
%\item First item
%\item Second item
%\squishend     %% \end{itemize}

\newcommand{\denselist}{\itemsep 0pt\topsep-6pt\partopsep-6pt}


\newtheorem{thm}{Theorem}[section]
\newtheorem{cor}{Corollary}[section]
\newtheorem{defn}{Definition}[section]
\newenvironment{mythm}{{\bf Theorem}}{}



\newcommand{\tm}{\tilde{m}}
\newcommand{\tv}{\tilde{v}}

% For bold vector symbols
\newcommand{\myvec}[1]{\boldsymbol{#1}}
\newcommand{\myvecsym}[1]{\boldsymbol{#1}}
\newcommand{\ind}[1]{\mathbb{I}(#1)}

\newcommand{\vzero}{\myvecsym{0}}
\newcommand{\vone}{\myvecsym{1}}
\newcommand{\valpha}{\myvecsym{\alpha}}
\newcommand{\vbeta}{\myvecsym{\beta}}
\newcommand{\vchi}{\myvecsym{\chi}}
\newcommand{\vdelta}{\myvecsym{\delta}}
\newcommand{\vDelta}{\myvecsym{\Delta}}
\newcommand{\vepsilon}{\myvecsym{\epsilon}}
\newcommand{\vell}{\myvecsym{\ell}}
\newcommand{\veta}{\myvecsym{\eta}}
\newcommand{\vgamma}{\myvecsym{\gamma}}
\newcommand{\vGamma}{\myvecsym{\Gamma}}
\newcommand{\vmu}{\myvecsym{\mu}}
\newcommand{\vnu}{\myvecsym{\nu}}
\newcommand{\vkappa}{\myvecsym{\kappa}}
\newcommand{\vlambda}{\myvecsym{\lambda}}
\newcommand{\vLambda}{\myvecsym{\Lambda}}
\newcommand{\vLambdaBar}{\overline{\vLambda}}
\newcommand{\vomega}{\myvecsym{\omega}}
\newcommand{\vOmega}{\myvecsym{\Omega}}
\newcommand{\vphi}{\myvecsym{\phi}}
\newcommand{\vPhi}{\myvecsym{\Phi}}
\newcommand{\vpi}{\myvecsym{\pi}}
\newcommand{\vpsi}{\myvecsym{\psi}}
\newcommand{\vPsi}{\myvecsym{\Psi}}
\newcommand{\vtheta}{\myvecsym{\theta}}
\newcommand{\vTheta}{\myvecsym{\Theta}}
\newcommand{\vsigma}{\myvecsym{\sigma}}
\newcommand{\vSigma}{\myvecsym{\Sigma}}
\newcommand{\vtau}{\myvecsym{\tau}}
\newcommand{\vupsilon}{\myvecsym{\upsilon}}
\newcommand{\vxi}{\myvecsym{\xi}}

\newcommand{\vxn}{\vx^{(n)}}

\newcommand{\vmuY}{\vb}
\newcommand{\vmuMu}{\vmu_{x}}
\newcommand{\vmuMuGivenY}{\vmu_{x|y}}
\newcommand{\vSigmaMu}{\vSigma_{x}}
\newcommand{\vSigmaMuInv}{\vSigma_{x}^{-1}}
\newcommand{\vSigmaMuGivenY}{\vSigma_{x|y}}
\newcommand{\vSigmaMuGivenYinv}{\vSigma_{x|y}^{-1}}
\newcommand{\vSigmaY}{\vSigma_{y}}
\newcommand{\vSigmaYinv}{\vSigma_{y}^{-1}}

%\newcommand{\vmuY}{\vmu_{y}}
%\newcommand{\vmuMu}{\vmu_{\mu}}
%\newcommand{\vmuMuGivenY}{\vmu_{\mu|y}}
%\newcommand{\vSigmaMu}{\vSigma_{\mu}}
%\newcommand{\vSigmaMuInv}{\vSigma_{\mu}^{-1}}
%\newcommand{\vSigmaMuGivenY}{\vSigma_{\mu|y}}
%\newcommand{\vSigmaMuGivenYinv}{\vSigma_{\mu|y}^{-1}}
%\newcommand{\vSigmaY}{\vSigma_{y}}
%\newcommand{\vSigmaYinv}{\vSigma_{y}^{-1}}

\newcommand{\muY}{\mu_{y}}
\newcommand{\muMu}{\mu_{\mu}}
\newcommand{\muMuGivenY}{\mu_{\mu|y}}
\newcommand{\SigmaMu}{\Sigma_{\mu}}
\newcommand{\SigmaMuInv}{\Sigma_{\mu}^{-1}}
\newcommand{\SigmaMuGivenY}{\Sigma_{\mu|y}}
\newcommand{\SigmaMuGivenYinv}{\Sigma_{\mu|y}^{-1}}
\newcommand{\SigmaY}{\Sigma_{y}}
\newcommand{\SigmaYinv}{\Sigma_{y}^{-1}}

\newcommand{\hatf}{\hat{f}}
\newcommand{\haty}{\hat{y}}
\newcommand{\const}{\mbox{const}}
\newcommand{\sigmoid}{\mbox{sigm}}

\newcommand{\one}{(1)}
\newcommand{\two}{(2)}

\newcommand{\va}{\myvec{a}}
\newcommand{\vb}{\myvec{b}}
\newcommand{\vc}{\myvec{c}}
\newcommand{\vd}{\myvec{d}}
\newcommand{\ve}{\myvec{e}}
\newcommand{\vf}{\myvec{f}}
\newcommand{\vg}{\myvec{g}}
\newcommand{\vh}{\myvec{h}}
\newcommand{\vj}{\myvec{j}}
\newcommand{\vk}{\myvec{k}}
\newcommand{\vl}{\myvec{l}}
\newcommand{\vm}{\myvec{m}}
\newcommand{\vn}{\myvec{n}}
\newcommand{\vo}{\myvec{o}}
\newcommand{\vp}{\myvec{p}}
\newcommand{\vq}{\myvec{q}}
\newcommand{\vr}{\myvec{r}}
\newcommand{\vs}{\myvec{s}}
\newcommand{\vt}{\myvec{t}}
\newcommand{\vu}{\myvec{u}}
\newcommand{\vv}{\myvec{v}}
\newcommand{\vw}{\myvec{w}}
\newcommand{\vws}{\vw_s}
\newcommand{\vwh}{\hat{\vw}}
\newcommand{\vx}{\myvec{x}}
%\newcommand{\vx}{\myvec{x}}
\newcommand{\vxt}{\myvec{\tilde{x}}}
\newcommand{\vy}{\myvec{y}}
\newcommand{\vyt}{\myvec{\tilde{y}}}
\newcommand{\vz}{\myvec{z}}

\newcommand{\vA}{\myvec{A}}
\newcommand{\vB}{\myvec{B}}
\newcommand{\vC}{\myvec{C}}
\newcommand{\vD}{\myvec{D}}
\newcommand{\vE}{\myvec{E}}
\newcommand{\vF}{\myvec{F}}
\newcommand{\vG}{\myvec{G}}
\newcommand{\vH}{\myvec{H}}
\newcommand{\vI}{\myvec{I}}
\newcommand{\vJ}{\myvec{J}}
\newcommand{\vK}{\myvec{K}}
\newcommand{\vL}{\myvec{L}}
\newcommand{\vM}{\myvec{M}}
\newcommand{\vN}{\myvec{N}}
\newcommand{\vO}{\myvec{O}}
\newcommand{\vP}{\myvec{P}}
\newcommand{\vQ}{\myvec{Q}}
\newcommand{\vR}{\myvec{R}}
\newcommand{\vS}{\myvec{S}}
\newcommand{\vT}{\myvec{T}}
\newcommand{\vU}{\myvec{U}}
\newcommand{\vV}{\myvec{V}}
\newcommand{\vW}{\myvec{W}}
\newcommand{\vX}{\myvec{X}}
%\newcommand{\vXs}{\vX_{\vs}}
\newcommand{\vXs}{\vX_{s}}
\newcommand{\vXt}{\myvec{\tilde{X}}}
\newcommand{\vY}{\myvec{Y}}
\newcommand{\vZ}{\myvec{Z}}


\newcommand{\vxtest}{\myvec{x}_*}
\newcommand{\vytest}{\myvec{y}_*}


\newcommand{\ftrue}{f_{true}}

\newcommand{\myprec}{\mbox{prec}}
\newcommand{\precw}{\lambda_{w}} % precision of weights (alpha)
\newcommand{\precy}{\lambda_{y}} % precision of y (beta)
\newcommand{\fbar}{\overline{f}}
\newcommand{\xmybar}{\overline{x}}
\newcommand{\ybar}{\overline{y}}
\newcommand{\zbar}{\overline{z}}
\newcommand{\vxbar}{\overline{\vx}}
\newcommand{\vXbar}{\overline{\vX}}
\newcommand{\vybar}{\overline{\vy}}
\newcommand{\vYbar}{\overline{\vY}}
\newcommand{\vzbar}{\overline{\vz}}
\newcommand{\vZbar}{\overline{\vZ}}
\newcommand{\xbar}{\overline{x}}
\newcommand{\Xbar}{\overline{X}}
\newcommand{\Ybar}{\overline{Y}}
\newcommand{\Gbar}{\overline{G}}
\newcommand{\Jbar}{\overline{J}}
\newcommand{\Lbar}{\overline{L}}
\newcommand{\Nbar}{\overline{N}}
%\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Qbar}{\overline{Q}}
\newcommand{\Tbar}{\overline{T}}
\newcommand{\Sbar}{\overline{S}}
\newcommand{\vSbar}{\overline{\vS}}
\newcommand{\Rbar}{\overline{R}}

\newcommand{\vtaubar}{\overline{\vtau}}
\newcommand{\vtbar}{\overline{\vt}}
\newcommand{\vsbar}{\overline{\vs}}

\newcommand{\htilde}{\tilde{h}}
\newcommand{\vhtilde}{\tilde{\vh}}
\newcommand{\Dtilde}{\tilde{D}}
\newcommand{\Ftilde}{\tilde{F}}
\newcommand{\wtilde}{\tilde{w}}
\newcommand{\ptilde}{\tilde{p}}
\newcommand{\pemp}{p_{emp}}
\newcommand{\pstar}{p^*}
\newcommand{\xtilde}{\tilde{x}}
\newcommand{\Xtilde}{\tilde{X}}
\newcommand{\ytilde}{\tilde{y}}
\newcommand{\Ytilde}{\tilde{Y}}
\newcommand{\vxtilde}{\tilde{\vx}}
\newcommand{\vytilde}{\tilde{\vy}}
\newcommand{\ztilde}{\tilde{\z}}
\newcommand{\vztilde}{\tilde{\vz}}
\newcommand{\vthetaMAP}{\hat{\vtheta}_{MAP}}
\newcommand{\vthetaS}{\vtheta^{(s)}}
\newcommand{\vthetahat}{\hat{\vtheta}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\overline{\theta}}
\newcommand{\vthetabar}{\overline{\vtheta}}
\newcommand{\pibar}{\overline{\pi}}
\newcommand{\vpibar}{\overline{\vpi}}


%\newcommand{\subsubsubsection}[1]{\paragraph{#1}}
\newcommand{\choice}[2]{\left(\!\!\! \begin{array}{c} #1 \\ #2\end{array} \!\!\!\right)}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\defeq}{\stackrel{\rm def}{=}}
\newcommand{\real}{\mathbb{R}}

\newcommand{\given}{\|}
\newcommand{\indep}[2]{{#1} \perp {#2}}
\newcommand{\condindep}[3]{{#1} \perp {#2} | {#3}}
\newcommand{\condindepG}[3]{{#1} \perp_G {#2} | {#3}}
\newcommand{\condindepP}[3]{{#1} \perp_p {#2} | {#3}}
\newcommand{\depend}[2]{{#1} \not \perp {#2}}
\newcommand{\conddepend}[3]{{#1} \not \perp {#2} | {#3}}

\newcommand{\trans}[1]{{#1}^{\mathtt{T}}}
\newcommand{\inv}[1]{{#1}^{-1}}

\newcommand{\ra}{\rightarrow}
\newcommand{\lra}{\leftrightarrow}
\newcommand{\Ra}{\Rightarrow}
%\newcommand{\rv}{r.v.}
\newcommand{\la}{\leftarrow}
\newcommand{\tr}{\mbox{tr}}
\newcommand{\st}{\mbox{  s.t.  }}

\newcommand{\dom}{\mbox{dom}}
\newcommand{\bel}{\mbox{bel}}
\newcommand{\dsep}{\mbox{dsep}}
\newcommand{\sep}{\mbox{sep}}
\newcommand{\entails}{\models}
\newcommand{\range}{\mbox{range}}
\newcommand{\myspan}{\mbox{span}}
\newcommand{\nullspace}{\mbox{nullspace}}
\newcommand{\adj}{\mbox{adj}}

\newcommand{\nbd}{\mbox{nbd}}
\newcommand{\nbr}{\mbox{nbr}}
\newcommand{\anc}{\mbox{anc}}
\newcommand{\desc}{\mbox{desc}}
\newcommand{\pred}{\mbox{pred}}
\newcommand{\nondesc}{\mbox{nondesc}}
\newcommand{\pa}{\pi}
\newcommand{\ch}{\mbox{ch}}
\newcommand{\mb}{\mbox{mb}}
\newcommand{\connects}{\sim}


\newcommand{\betadist}{\mbox{Beta}}
\newcommand{\Betadist}{\mbox{Beta}}
\newcommand{\bernoulli}{\mbox{Ber}}
\newcommand{\Ber}{\mbox{Ber}}
\newcommand{\Binom}{\mbox{Bin}}
\newcommand{\NegBinom}{\mbox{NegBinom}}
\newcommand{\binomdist}{\mbox{Bin}}
\newcommand{\cauchy}{\mbox{Cauchy}}
\newcommand{\DE}{\mbox{DE}}
\newcommand{\Dir}{\mbox{Dir}}
\newcommand{\discrete}{\calM}
\newcommand{\Discrete}{\calM}
\newcommand{\expdist}{\mbox{Exp}}
\newcommand{\expon}{\mbox{Expon}}
\newcommand{\gammadist}{\mbox{Ga}}
\newcommand{\Ga}{\mbox{Ga}}
\newcommand{\gauss}{{\cal N}}
\newcommand{\IG}{\mbox{IG}}
\newcommand{\IGauss}{\mbox{InvGauss}}
\newcommand{\IW}{\mbox{IW}}
\newcommand{\Laplace}{\mbox{Lap}}
\newcommand{\Mu}{\mbox{Mu}}
\newcommand{\Multi}{\mbox{Mu}}
\newcommand{\NIX}{NI\chi^2}
\newcommand{\GIX}{NI\chi^2}
\newcommand{\NIG}{\mbox{NIG}}
\newcommand{\GIG}{\mbox{NIG}}
\newcommand{\NIW}{\mbox{NIW}}
\newcommand{\GIW}{\mbox{NIW}}
\newcommand{\MVNIW}{\mbox{NIW}}
\newcommand{\NW}{\mbox{NWi}}
\newcommand{\MVNIG}{\mbox{NIG}}
\newcommand{\NGdist}{\mbox{NG}}
\newcommand{\prob}{p}
\newcommand{\Poi}{\mbox{Poi}}
\newcommand{\Student}{{\cal T}}
\newcommand{\student}{{\cal T}}
\newcommand{\Wishart}{\mbox{Wi}}
\newcommand{\Wi}{\mbox{Wi}}
\newcommand{\unif}{\mbox{U}}
\newcommand{\etr}{\mbox{etr}}

\newcommand{\softmax}{\calS}
\newcommand{\soft}{\mbox{soft}}
\newcommand{\cond}{\mbox{cond}}
\newcommand{\sign}{\mbox{sign}}
\newcommand{\sgn}{\mbox{sgn}}
\newcommand{\iid}{\mbox{iid}}
\newcommand{\mle}{\mbox{mle}}
\newcommand{\myiff}{\mbox{iff}}
\newcommand{\pd}{\mbox{pd}}
\newcommand{\pdf}{\mbox{pdf }}
\newcommand{\cdf}{\mbox{cdf}}
\newcommand{\pmf}{\mbox{pmf}}
\newcommand{\wrt}{\mbox{wrt}}
\newcommand{\matlab}{{\sc MATLAB}}
\newcommand{\NETLAB}{{\sc NETLAB}}
\newcommand{\MLABA}{\mbox{PMTK}}
\newcommand{\BLT}{\mbox{PMTK}}
\newcommand{\PMTK}{\mbox{PMTK}}
\newcommand{\mywp}{\mbox{wp}}

\newcommand{\KLpq}[2]{\mathrm{KL}\left[{#1}\|{#2}\right]}
\newcommand{\KL}{\mbox{KL}}
\newcommand{\MI}{\mathbb{I}}
\newcommand{\MIxy}[2]{\mathbb{I}\left({#1};{#2}\right)}
\newcommand{\MIxyz}[3]{\mathbb{I}\left({#1};{#2}|{#3}\right)}
\newcommand{\entropy}[1]{\mathbb{H}\left({#1}\right)}
\newcommand{\entropypq}[2]{\mathbb{H}\left({#1}, {#2}\right)}


\newcommand{\vvec}{\mbox{vec}}
\newcommand{\kron}{\otimes}
\newcommand{\dof}{\mbox{dof}}
%\newcommand{\E}{E}
\newcommand{\E}{\mathbb{E}}
\newcommand{\energy}{E}
\newcommand{\expectAngle}[1]{\langle #1 \rangle}
%\newcommand{\expect}[1]{\mathbb{E}\left[ {#1} \right]}
\newcommand{\expect}[2]{\mathds{E}_{{#1}} \left[ {#2} \right]}
\newcommand{\expectGiven}[3]{\mathds{E}_{{#1}} \left[ {#2} \mid {#3} \right]}
\newcommand{\Var}{\mbox{Var}}
\newcommand{\VarGiven}[3]{\mbox{Var}_{{#1}}\left[ {#2} \mid {#3}\right]}
%\newcommand{\Var}{\mathbb{V}}
\newcommand{\var}[1]{\mbox{var}\left[{#1}\right]}
\newcommand{\std}[1]{\mbox{std}\left[{#1}\right]}
\newcommand{\varQ}[2]{\mbox{var}_{{#2}}\left[{#1}\right]}
\newcommand{\cov}[1]{\mbox{cov}\left[{#1}\right]}
%\newcommand{\mode}[1]{\mbox{mode}\left[{#1}\right]}
\newcommand{\median}[1]{\mbox{median}\left[{#1}\right]}



\newcommand{\diag}{\mbox{diag}}
\newcommand{\blkdiag}{\mbox{blkdiag}}
\newcommand{\bias}{\mbox{bias}}
\newcommand{\union}{\cup}
\newcommand{\intersect}{\cap}

\newcommand{\size}{\mbox{size}}
\newcommand{\trace}{\mbox{trace}}


\newcommand{\myc}{c}
\newcommand{\myi}{i}
\newcommand{\myj}{j}
\newcommand{\myk}{k}
\newcommand{\myn}{n}
\newcommand{\myq}{q}
\newcommand{\mys}{s}
\newcommand{\myt}{t}


\newcommand{\supp}{\mbox{supp}}


\newcommand{\calA}{{\cal A}}
\newcommand{\calB}{{\cal B}}
\newcommand{\calC}{{\cal C}}
\newcommand{\calD}{{\cal D}}
\newcommand{\calDx}{{\cal D}_x}
\newcommand{\calE}{{\cal E}}
\newcommand{\cale}{{\cal e}}
\newcommand{\calF}{{\cal F}}
\newcommand{\calG}{{\cal G}}
\newcommand{\calH}{{\cal H}}
\newcommand{\calHX}{{\cal H}_X}
\newcommand{\calHy}{{\cal H}_y}
\newcommand{\calI}{{\cal I}}
\newcommand{\calK}{{\cal K}}
\newcommand{\calM}{{\cal M}}
\newcommand{\calN}{{\cal N}}
\newcommand{\caln}{{\cal n}}
\newcommand{\calNP}{{\cal NP}}
\newcommand{\calMp}{\calM^+}
\newcommand{\calMm}{\calM^-}
\newcommand{\calMo}{\calM^o}
\newcommand{\Ctest}{C_*}
\newcommand{\calL}{{\cal L}}
\newcommand{\calP}{{\cal P}}
\newcommand{\calq}{{\cal q}}
\newcommand{\calQ}{{\cal Q}}
\newcommand{\calR}{{\cal R}}
\newcommand{\calS}{{\cal S}}
\newcommand{\calSstar}{\calS_*}
\newcommand{\calT}{{\cal T}}
\newcommand{\calV}{{\cal V}}
\newcommand{\calv}{{\cal v}}
\newcommand{\calX}{{\cal X}}
\newcommand{\calY}{{\cal Y}}

\newcommand{\Lone}{$\ell_1$}
\newcommand{\Ltwo}{$\ell_2$}

\newcommand{\mya}{\mbox{a}}
\newcommand{\myat}{\alpha_{t|t-1}}
\newcommand{\score}{\mbox{score}}
\newcommand{\AIC}{\mbox{AIC}}
\newcommand{\BIC}{\mbox{BIC}}
\newcommand{\BICcost}{\mbox{BIC-cost}}
\newcommand{\scoreBIC}{\mbox{score-BIC}}
\newcommand{\scoreBICL}{\mbox{score-BIC-L1}}
\newcommand{\scoreL}{\mbox{score-L1}}

\newcommand{\ecoli}{\mbox{{\it E. coli}}}
\newcommand{\doPearl}{\mbox{do}}
\newcommand{\data}{\calD}
\newcommand{\model}{\calM}
\newcommand{\dataTrain}{\calD_{\mbox{train}}}
\newcommand{\dataTest}{\calD_{\mbox{test}}}
\newcommand{\dataValid}{\calD_{\mbox{valid}}}
\newcommand{\futuredata}{\tilde{\calD}}
\newcommand{\algo}{\calA}
\newcommand{\fitAlgo}{\calF}
\newcommand{\predictAlgo}{\calP}
\newcommand{\err}{\mbox{err}}
\newcommand{\logit}{\mbox{logit}}
\newcommand{\parent}{\mbox{pa}}


%%%%%%%%%%% Hoyt

\newcommand{\conv}[1]{\,\,\,\displaystyle{\operatorname*{\longrightarrow}^{\,_{#1}\,}}\,\,\,}
\newcommand{\dconv}{\conv{D}}
\newcommand{\pconv}{\conv{P}}
\newcommand{\asconv}{\conv{AS}}
\newcommand{\lpconv}[1]{\conv{L^{#1}}}

\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{n}


\newcommand{\condSet}{\mathcal{S}}
\newcommand{\condSetC}{\mathcal{\lnot S}}



==> section/gold.tex <==
\section{International Mathematical Olympiad (IMO)}

We follow the generate--verify--refine test-time scaling pipeline of prior work~\citep{shao2025deepseekmathv2selfverifiablemathematicalreasoning} and allocate a large inference-time compute budget to evaluate Loopie-20B-A2B on the 2025 IMO problems. For each problem, we initialize a candidate pool with 64 independently generated solutions and sample 64 verification analyses for each candidate. We rank the candidates according to their average verification scores and retain the top 64 solutions. For each retained solution, we sample eight verification analyses, prioritizing critiques that identify concrete errors, logical gaps, or missing justifications, and use the resulting solution--critique pairs to generate refined solutions. The refined solutions are added back to the candidate pool. This procedure is repeated for up to 16 iterations, with early termination when a candidate passes all 64 verification attempts. Finally, we select the solution with the highest aggregated verification score for evaluation, Each question was scored by GPT-5.5 acting as an LLM-as-a-judge. The evaluation was repeated three times, and the average score was reported. Further details are provided in Appendix E.

\begin{table}[H]
  \centering
  \captionsetup{type=table,hypcap=false}
  \caption{Performance on IMO 2025. The gold, silver, and bronze medal thresholds are 35, 28, and 19 points.
  }
  \setlength{\tabcolsep}{5.8pt}
  \renewcommand{\arraystretch}{1.0}
  \small

  \begin{tabular}{@{}lccccccc@{}}
  \toprule
  \multicolumn{8}{c}{\textbf{IMO 2025}} \\
  \midrule
  \textbf{\textcolor{iclrdeepblue}{Loopie-20B-A2B} w/ TTS}
    & $7$
    & $7$
    & $4$
    & $6$
    & $7$
    & $4$
    & $35$\,\goldmedalicon \\
  \bottomrule
  \end{tabular}
\end{table}

\section{International Physics Olympiad (IPhO)}
Following the generate--verify--refine pipeline used for IMO, we apply a similar generate--vote--critic test-time scaling strategy to the IPhO problems. Our procedure largely follows prior work~\citep{su01}, while allocating additional refinement rounds to accommodate the longer reasoning chains and more involved calculations required in physics problems. With extensive test-time scaling, Loopie-20B-A2B achieved a gold-medal-level score of 20.3 on the IPhO, surpassing the gold medal threshold of 19.7 points.

==> tables/dolmino_sample.tex <==
\begin{table}[h]
\centering
\newcolumntype{E}{>{\columncolor{lightgrey}}c}
\newcolumntype{Q}{>{\columncolor{ai2offwhite}}c}
\newcolumntype{D}{>{\columncolor{ai2lightpink}}c}
\adjustbox{max width=\linewidth}{
\begin{tabular}{l@{\hspace{.2em}}c E E Q Q D D}
\toprule
    \multirow{2}{*}{\textbf{Source}} & 
    \multirow{2}{*}{\textbf{Tokens}} & 
    \multicolumn{2}{>{\columncolor{midgrey}}c}{\textbf{50B}} &
    \multicolumn{2}{>{\columncolor{ai2midwhite}}c}{\textbf{100B}} &
    \multicolumn{2}{>{\columncolor{ai2midpink}}c}{\textbf{300B}} 
\\
    \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} 
    & 
    & 
    \multicolumn{1}{>{\columncolor{midgrey}}c}{\textbf{Source \%}} & 
    \multicolumn{1}{>{\columncolor{midgrey}}c}{\textbf{Mix \%}} &
    \multicolumn{1}{>{\columncolor{ai2midwhite}}c}{\textbf{Source \%}} & 
    \multicolumn{1}{>{\columncolor{ai2midwhite}}c}{\textbf{Mix \%}} & 
    \multicolumn{1}{>{\columncolor{ai2midpink}}c}{\textbf{Source \%}} & 
    \multicolumn{1}{>{\columncolor{ai2midpink}}c}{\textbf{Mix \%}} 
\\
\midrule
Filtered DCLM & 752B & 3.23 & 47.2 & 6.85 & 50.2 & 20.78 & 51.9 \\
Decontam. FLAN & 17.0B & 50.0 & 16.6 & 100 & 16.7 & 200 & 11.3 \\
StackExchange Q\&A & 1.26B & 100 & 2.45 & 200 & 2.47 & 400 & 1.68 \\
peS2o & 58.6B & 5.15 & 5.85 & 16.7 & 9.52 & 100 & 19.4 \\
Wikipedia/Wikibooks & 3.7B & 100 & 7.11 & 100 & 3.57 & 400 & 4.86 \\
Dolmino Math & 10.7B & 100 & 20.8 & 200 & 17.5 & 400 & 10.8 \\
\bottomrule
\end{tabular}
}
\vspace{3pt}
\caption{\dolminos compositions. The Source \% column indicates the fraction of the source that was used in the \textsc{Dolmino} mix. Numbers in this column greater than 100 indicate we used the data, e.g. 400 indicates a 4x repeat. The Mix \% column describes the proportion of the \textsc{Dolmino} mix that is composed of this source, i.e., this column should sum to 100\%.}
\label{tab:dolmino-composition-pretty}
\end{table}


==> tables/environmental_impact.tex <==

\begin{table}[h]
\centering
\adjustbox{max width=\linewidth}{
\begin{tabular}{l c c c c c c c c c}
\toprule
\textbf{Model} & \textbf{\makecell{Total GPU\\Power (MWh)}} & \textbf{\makecell{Power Usage\\Effect.}} & \textbf{\makecell{Carbon\\Intensity}} & \textbf{\makecell{Carbon\\Emissions}} & \textbf{\makecell{Water Usage\\Effect.}} & \textbf{\makecell{Total Water\\Usage (kL)}} \\
\midrule
Llama 2 7B & 74 & 1.1 & - & 31 & \underline{1.29 - 4.26} & \underline{105 - 347} \\
Llama 3.1 8B & 1,022 & 1.1 & - & 420 & \underline{1.29 - 4.26} & \underline{1,450 - 4,823} \\
\rowcolor{ai2offwhite}OLMo 7B & 104 & 1.1 & 0.610 & 70 & 4.26 & 487 \\
\rowcolor{ai2lightpink}\olmotoo 7B & 131 & 1.2 & 0.332 & 52 & 1.29 & 202 \\
\rowcolor{ai2lightpink}\olmotoo 13B & 257 & 1.12 & 0.351 & 101 & 3.10 & 892 \\
\bottomrule
\end{tabular}
}
\vspace{3pt}
\caption{CO\textsubscript{2} emissions and water consumption during pretraining. We estimate the total carbon emissions and water consumption for our new models using PUE information from our data center providers, carbon intensity data and WUE from the local grid for each data center, and total power consumption from time series data logged throughout training. Numbers for Llama 2 \citep{touvron2023llama}, Llama 3 \citep{dubey2024llama}, and the original OLMo \citep{Groeneveld2024OLMoAT} are taken from their respective papers. We also show {\bf simulated} water consumption for Llama 2 and 3, showing a range of water usage numbers using the lowest and highest WUE values for OLMo models.}
\label{tab:environmental_impact}
\end{table}


==> tables/eval-post.tex <==
\begin{table}[h]
\centering
\setlength\tabcolsep{5pt}
\begin{small}
\adjustbox{max width=\linewidth}{
\begin{tabular}{{@{}ll C{0.7cm} R{1.4cm} C{1cm} C{2cm} c@{}}}
\toprule
 \textbf{Category} & \textbf{Benchmark} & \textbf{CoT} & \textbf{\# Shots} & \textbf{Chat} & \textbf{Multiturn ICL} & \textbf{Metric} \\\midrule
\rowcolor{ai2offwhite}  Knowledge Recall & MMLU & \cmark & 0 & \cmark & \xmark & EM \\
\rowcolor{ai2offwhite} & PopQA & \xmark & 15 & \cmark & \cmark & EM \\
\rowcolor{ai2offwhite} & TruthfulQA & \xmark & 6 & \cmark & \xmark & MC2 \\
  Reasoning & BigBenchHard & \cmark & 3 & \cmark & \cmark & EM \\
  & DROP & \xmark & 3 & \xmark & N/A & F1 \\
\rowcolor{ai2offwhite}  Math & GSM8K & \cmark & 8 & \cmark & \cmark & EM \\
\rowcolor{ai2offwhite}   & MATH & \cmark & 4 & \cmark & \cmark & Flex EM \\
   Instruction Following & IFEval & \xmark & 0 & \cmark & N/A & Pass@1 (prompt; loose) \\
  & AlpacaEval 2 & \xmark & 0 & \cmark & N/A & LC Winrate \\
 \rowcolor{ai2offwhite}  Safety & \tulu Safety & \xmark & 0 & \cmark & N/A & Average$^*$ \\
\bottomrule
\end{tabular}}
\end{small}
\vspace{3pt}
\caption{
The \olmotoo Instruct Evaluation Regime (Adapted from \citet{lambert2024tulu3}): settings for development ({\bf{top}}) and unseen ({\bf{bottom}}) portions of the evaluation suite. {\bf{CoT}} are evaluations run with chain of thought prompting~\citep{wei2022chain}.
{\bf{\# shots}} is the number of in-context examples in the evaluation template.
{\bf{Chat}} indicates whether we use a chat template while prompting the model.
{\bf{Multiturn ICL}} indicates that we present each in-context example as a separate turn in a conversation (applicable only when a chat template is used and \# Shots is not 0).
$^*$Average over multiple sub-evaluations---full details of the safety evaluation are in \citet{lambert2024tulu3}.
}
\label{tab:eval-post}
\end{table}


==> tables/hypers-post.tex <==



\begin{table}[h]
\centering
\begin{minipage}{0.48\textwidth}
    \footnotesize
    \centering
    \setlength\tabcolsep{3pt}
    \begin{tabular}{>{\raggedright}p{0.35\linewidth}p{0.55\linewidth}}
        \toprule
        \textbf{Hyperparameter} & \textbf{RLVR value}  \\
        \midrule
        \rowcolor{ai2offwhite} Learning rate & $3 \cdot 10^{-7}$ for 13B; $4 \cdot 10^{-7}$ for 7B \\
        \rowcolor{ai2offwhite} Effective batch size & 248 for 13B; 224 for 7B \\
        \rowcolor{ai2offwhite} 
        KL penalty coef.  ($\beta$) &
        {0.1 for first and final 13B; 0.03 for second 13B; 0.05 for 7B} \\
        \rowcolor{ai2offwhite} Max total episodes & 200,000 for 13B; 100,000 for 7B \\
        Discount factor $\gamma$ & 1.0 \\
        General advantage estimation $\lambda$ & 0.95 \\
        Mini-batches $N_\text{mb}$ & 1 \\
        PPO update iterations $K$ & 4 \\
        \bottomrule
    \end{tabular}
\end{minipage}
\hfill
\begin{minipage}{0.48\textwidth}
    \footnotesize
    \centering
    \setlength\tabcolsep{3pt}
    \begin{tabular}{>{\raggedright}p{0.60\linewidth}p{0.3\linewidth}}
        \toprule
        \textbf{Hyperparameter} & \textbf{RLVR value}  \\
        \midrule
        PPO's clipping coefficient $\varepsilon$  & 0.2 \\
        Value function coefficient $c_1$ & 0.1 \\
        Gradient norm threshold & 1.0 \\
        Learning rate schedule & \textit{linear} \\
        Generation temperature & 1.0 \\
        Max token length & 2,048 \\
        Max prompt token length & 2,048 \\
        {Penalty reward for no EOS token} & $-10.0$ \\
        Response length & 2,048 \\
        Warm up ratio ($\omega$) & 0.0 \\
        \bottomrule
    \end{tabular}
\end{minipage}
\sethlcolor{ai2offwhite} %
\caption{The hyperparameters of PPO used for optimizing against the verifiable reward function with RLVR.
Hyparameters with different settings for the 7B and 13B parameter models are \hl{highlighted}.}
\label{tab:hypers_rlvr}
\end{table}




==> tables/instruct-stages.tex <==

\begin{table}[t]
\centering
\setlength\tabcolsep{3pt}
{\footnotesize
\begin{tabular}{lccccccccccc}
\toprule
    & 
    \textbf{AVG} & 
    \textbf{AE2} & 
    \textbf{BBH} & 
    \textbf{DROP} & 
    \textbf{GSM8K} & 
    \textbf{IFE} & 
    \textbf{MATH} & 
    \textbf{MMLU} & 
    \textbf{Safety} & 
    \textbf{PQA} & 
    \textbf{TQA} \\
\midrule
OLMo 2 1B SFT & 36.9 & 2.4 & 32.8 & 33.8 & 52.1 & 50.5 & 13.2 & 36.4 & \bf{93.2} & 12.7 & 42.1 \\

\rowcolor{ai2offwhite} OLMo 2 1B DPO & 40.6 & \bf{9.5} & 33.0 & 34.5 & 59.0 & 67.1 & 14.1 & 39.9 & 89.9 & 12.3 & 46.4 \\

\rowcolor{ai2lightpink} OLMo 2 1B Instruct & \bf{42.7} & 9.1 & \bf{35.0} & \bf{34.6} & \bf{68.3} & \bf{70.1} & \bf{20.7} & \bf{40.0} & 87.6 & \bf{12.9} & \bf{48.7}
\\\midrule

OLMo 2 7B SFT & 51.4 & 10.2   & 49.6 & 59.6 & 74.6 & 66.9 & 25.3 & 61.1 & \bf{94.6} & \bf{23.6} & 48.6 \\
\rowcolor{ai2offwhite} OLMo 2 7B DPO & 55.9 & 27.9 & 51.1   & 60.2 & 82.6 & \bf{73.0} & 30.3 & 60.8 & 93.7 & 23.5 & 56.0 \\
 \rowcolor{ai2lightpink}   OLMo 2 7B Instruct & \bf{56.5} & \bf{29.1}   & \bf{51.4} & \bf{60.5} & \bf{85.1} & 72.3 & \bf{32.5} & \bf{61.3} & 93.3 & 23.2 & \bf{56.5} \\ \midrule
 OLMo 2 13B SFT & 56.6 & 11.5   & 59.9 & 71.3 & 76.3 & 68.6 & 29.5 & 68.0 & \bf{94.3} & \bf{29.4} & 57.1 \\
 \rowcolor{ai2offwhite}  OLMo 2 13B DPO & 62.0 & \bf{38.3} & 61.4 & 71.5 & 82.3 & \bf{80.2} & 35.2 & 67.9 & 90.3 & 29.0 & \bf{63.9} \\
 \rowcolor{ai2lightpink}  OLMo 2 13B Instruct & \bf{63.4} & 39.5 & \bf{63.0} & \bf{71.5} & \bf{87.4} & 82.6 & \bf{39.2} & \bf{68.5} & 89.7 & 28.8 & 64.3 \\ \midrule
 OLMo 2 32B SFT & 61.7 & 16.9 & 69.7 & 77.2 & 78.4 & 72.4 & 35.9 & 76.1 & \bf{93.8} & 35.4 & 61.3 \\
 \rowcolor{ai2offwhite} OLMo 2 32B DPO & \bf{68.8} & \bf{44.1} & 70.2 & 77.5 & 85.7 & 83.8 & 46.8 & \bf{78.0} & 91.9 & 36.4 & \bf{73.5} \\
 \rowcolor{ai2lightpink} OLMo 2 32B Instruct & \bf{68.8} & 42.8 & \bf{70.6} & \bf{78.0} & \bf{87.6} & \bf{85.6} & \bf{49.7} & 77.3 & 85.9 & \bf{37.5} & 73.2 \\
\bottomrule
\end{tabular}
}
\caption{Comparison of performance for OLMo 2 Instruct after different training stages. The final Instruct model is from the RLVR stage.
The following evaluation names are abbreviated: AVG -- Average, AE2 -- AlpacaEval 2, BBH -- BigBenchHard, IFE -- IFEval, PQA -- PopQA, TQA -- TruthfulQA.
}
\label{tab:instruct_stages}
\end{table}


==> tables/instruct-unseen.tex <==
\begin{table}[t]
\centering
\setlength\tabcolsep{3pt}
{\small
\begin{tabular}{l c c c c c c}
\hline
 &  & AGI Eval & DeepMind  &  &  & \\ 
Model & Average &  English &  Math & GPQA & IFEval OOD & MMLU Pro \\ \hline
OLMo 2 32B Instruct & 44.9 & 68.3 & 34.7 & 35.9 & 33.1 & 52.7 \\
OLMo 2 32B DPO & 43.8 & 68.6 & 34.5 & 35.7 & 26.8 & 53.3 \\
OLMo 2 32B SFT & 39.3 & 63.9 & 33.4 & 32.6 & 20.4 & 46.3 \\
OLMo 2 1124 13B Inst. & 35.2 & 60.5 & 26.8 & 28.8 & 18.7 & 41.4 \\
OLMo 2 1124 13B DPO & 35.5 & 60.1 & 25.4 & 32.1 & 18.0 & 41.8 \\
OLMo 2 1124 13B SFT & 33.0 & 56.0 & 27.1 & 27.0 & 16.6 & 38.2 \\
OLMo 2 1124 7B Inst. & 32.2 & 57.2 & 19.1 & 30.1 & 18.7 & 36.0 \\
OLMo 2 1124 7B DPO & 31.8 & 56.7 & 17.7 & 30.6 & 17.3 & 36.6 \\
OLMo 2 1124 7B SFT & 29.8 & 52.7 & 19.0 & 27.7 & 16.2 & 33.2 \\
OLMo 7B 0724 Inst. & 22.9 & 43.6 & 5.8 & 27.9 & 14.4 & 22.9 \\
OLMoE 1B 7B 0924 Inst. & 20.5 & 39.1 & 4.2 & 27.5 & 11.3 & 20.6 \\ \hline
\end{tabular}
}
\caption{Evaluation results for OLMo Instruct models on the unseen suite from~\citet{lambert2024tulu3}.
Note that IFEval OOD has been improved via minor bug fixes for OLMo 2 7B and 13B, so the numbers are not exactly comparable to those in~\citet{lambert2024tulu3}. }
\label{tab:instruct-unseen}
\end{table}


==> tables/instruct.tex <==






==> tables/microanneal.tex <==
\begin{table}[h]
\setlength\tabcolsep{10pt}
\begin{center}
\begin{small}
\begin{tabular}{lcccc}
\toprule
\rowcolor{midgrey}\multicolumn{5}{c}{\textbf{\textit{Microanneal Experiment 1}}} \\
\rowcolor{lightgrey}{\bf{Mix}} & {\bf{Web ratio}} & {\bf{Tokens}} & {\bf{MMLU}} (avg) & {\bf{GSM*}} \\
\rowcolor{lightgrey}Baseline & \textit{n/a} & \textit{n/a} & 59.8 & 28.5 \\
\rowcolor{lightgrey}Math 35/65 & 65.0\% & 576M & 60.1 & 63.5 \\
\rowcolor{lightgrey}Math 10/90 & 88.3\% & 1.72B & 60.9 & 61.0 \\
\midrule
\rowcolor{ai2midwhite}\multicolumn{5}{c}{\textbf{\textit{Microanneal Experiment 2}}} \\
\rowcolor{ai2offwhite}{\bf{Mix}} & {\bf{Web ratio}} & {\bf{Tokens}} & {\bf{MMLU}} (avg) & {\bf{GSM*}} \\
\rowcolor{ai2offwhite} Baseline & \textit{n/a} & \textit{n/a} & 59.8 & 28.5 \\
\rowcolor{ai2offwhite} 1x Math & 65.0\% & 576M & 60.1 & 63.5 \\
\rowcolor{ai2offwhite} 2x Math & 49.3\% & 798M & 60.3 & 66.0 \\
\rowcolor{ai2offwhite} 4x Math & 48.6\% & 1.57B & 60.5 & 65.0 \\
\midrule
\rowcolor{ai2midpink}\multicolumn{5}{c}{\textbf{\textit{Microanneal Experiment 3}}} \\
\rowcolor{ai2lightpink}{\bf{Mix}} & {\bf{Web ratio}} & {\bf{Tokens}} & {\bf{MMLU}} (avg) & {\bf{GSM*}} \\
\rowcolor{ai2lightpink}
\rowcolor{ai2lightpink} Baseline & \textit{n/a} & \textit{n/a} & 59.8 & 28.5 \\
\rowcolor{ai2lightpink} TinyGSM-Inline & 47.9\% & 3.17B & 60.4 & 25.0 \\
\rowcolor{ai2lightpink} TinyGSM-MIND & 52.1\% & 6.40B & 61.4 & 65.5 \\
\rowcolor{ai2lightpink} 2x TinyGSM-MIND & 51.3\% & 12.6B & 62.1 & 70.0 \\
\bottomrule
\end{tabular}
\end{small}
\vspace{2mm}
\caption{Results from microanneal experiments to \olmotoo math capabilities. 
We evaluate math/not-math mixture ratio, impact of repeating math tokens, and different math datasets.
We monitor average MMLU scores to ensure \olmotoo remains performant on knowledge intensive tasks.
}
\label{tab:microanneal_results-pretty}

\end{center}
\end{table}


==> tables/midtrain_mixes.tex <==
\newcommand{\MeBaseline}{{\sans{PT Mix}}\xspace}
\newcommand{\MeDclmSeven}{{\sans{Web }}$^{\text{{\sans{FT}}}_\text{{\sans{7}}}}$\xspace}
\newcommand{\MeFinewebThree}{{\sans{Web }}$^{\text{{\sans{FT}}}_\text{{\sans{7}}}}_{\text{{\sans{FW}}}_\text{{\sans{3}}}}$\xspace}
\newcommand{\MeFinewebTwo}{{\sans{Web }}$^{\text{{\sans{FT}}}_\text{{\sans{7}}}}_{\text{{\sans{FW}}}_\text{{\sans{2}}}}$\xspace}
\newcommand{\MeFinewebTwoMath}{{\sans{Web }}$^{\text{{\sans{FT}}}_\text{{\sans{7}}}}_{\text{{\sans{FW}}}_\text{{\sans{2}}}}${\sans + Math}\xspace}
\newcommand{\MeFinewebTwoIns}{{\sans{Web }}$^{\text{{\sans{FT}}}_\text{{\sans{7}}}}_{\text{{\sans{FW}}}_\text{{\sans{2}}}}${\sans + Ins}\xspace}
\newcommand{\MeFinewebTwoMathIns}{{\sans{Web }}$^{\text{{\sans{FT}}}_\text{{\sans{7}}}}_{\text{{\sans{FW}}}_\text{{\sans{2}}}}${\sans + Math + Ins}\xspace}


\begin{table}[ht]
\renewcommand{\arraystretch}{.9}
\setlength\tabcolsep{3pt}
\begin{center}
\begin{footnotesize}
\newcommand{\rot}[1]{\rotatebox{90}{#1}}
\begin{tabular}{c @{\hskip 6pt} l @{\hskip 6pt} l c c c c c c c}
\toprule
    & \multirow{2}{*}{\vspace{-1.5em}\textbf{\footnotesize{Source}}} 
    &
    & \multicolumn{7}{c}{\textbf{\footnotesize~Mix \%}} 
    \vspace{.5em}
    \\[-.3em]
    &
    &
    &
    \MeBaseline &
    \MeDclmSeven &
    \MeFinewebThree &
    \MeFinewebTwo &
    \makecell[lc]{
        \MeFinewebTwo
        \\[-.2em]
        {\sans{+ Math}}
    } &
    \makecell[lc]{
        \MeFinewebTwo
        \\[-.2em]
        {\sans{+ Ins}}
    } &
    \makecell[lc]{
        \MeFinewebTwo
        \\[-.2em]
        {\sans{+ Math}}
        \\[-.2em]
        {\sans{+ Ins}}
    }
    \\
\midrule
    \rowcolor{ai2offwhite}
    &
    \sans{DCLM} & 
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}from}
        \\[-.4em]
        {\scriptsize\color{darkergrey}pretrain}
    \end{tabular} & 
    95.2 & 
    - & 
    - & 
    - & 
    - & 
    - & 
    - 
\\
    \rowcolor{ai2offwhite}
    & 
    \sans{DCLM} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}FT top 7\%}\\
    \end{tabular} & 
    - &
    57.1 &
    - &
    - &
    - &
    - &
    -
\\
    \rowcolor{ai2offwhite}
    & 
    \sans{DCLM} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}FT top 7\%}
        \\[-.4em]
        {\scriptsize\color{darkergrey}$\text{FineWeb}\geqslant3$}
    \end{tabular} & 
    - &
    - &
    54.2 &
    - &
    - &
    - &
    -
\\
    \rowcolor{ai2offwhite}
    \multirow{-4}{*}{\rot{\textbf{\hspace{2em}\scriptsize{WEB}}}} & 
    \sans{DCLM} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}FT top 7\%}
        \\[-.4em]
        {\scriptsize\color{darkergrey}$\text{FineWeb}\geqslant2$}
    \end{tabular} & 
    - &
    - &
    - &
    57.9 &
    61.8 &
    75.5 &
    57.5
\\
    &
    \sans{Flan} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}Dolma 1.7}
        \\[-.4em]
        {\scriptsize\color{darkergrey}decontaminated}
    \end{tabular} & 
    - &
    - &
    - &
    - &
    - &
    8.8 &
    6.7
\\
    \multirow{-2}{*}{\rot{\textbf{\hspace{2em}\scriptsize{INST}}}} &
    \sans{Stack Exchange} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}2024/09/30 dump}
        \\[-.4em]
        {\scriptsize\color{darkergrey}Q\&A format}
    \end{tabular} & 
    - &
    - &
    - &
    - &
    - &
    0.7 &
    0.5
\\
    \rowcolor{ai2offwhite}
    &
    \sans{Starcoder} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}from}
        \\[-.4em]
        {\scriptsize\color{darkergrey}pretrain}
    \end{tabular} & 
    2.1 &
    19.5 &
    20.9 &
    19.2 &
    - &
    - &
    -
\\
    \rowcolor{ai2offwhite} 
    \multirow{-2}{*}{\rot{\hspace{2em}\textbf{\scriptsize{CODE}}}} &
    \sans{CodeSearchNet} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}unfiltered}\\
    \end{tabular} & 
    - &
    - &
    - &
    - &
    0.1 &
    0.2 &
    0.1
\\
    &
    \sans{Gutenberg Books} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}from}
        \\[-.4em]
        {\scriptsize\color{darkergrey}Dolma 1.7}
    \end{tabular} & 
    - &
    1.2 &
    1.3 &
    1.2 &
    - &
    - &
    -
\\
    &
    \sans{peS2o} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}from}
        \\[-.4em]
        {\scriptsize\color{darkergrey}pretrain}
    \end{tabular} & 
    1.5 &
    6.6 &
    7.1 &
    6.5 &
    10.7 &
    13.0 &
    9.9
\\
    &
    \sans{Wikipedia} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}from}
        \\[-.4em]
        {\scriptsize\color{darkergrey}pretrain}
    \end{tabular} & 
    0.1 &
    0.9 &
    0.9 &
    0.9 &
    1.6 &
    1.9 &
    1.4
\\
    &
    \sans{StackExchange} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}from}
        \\[-.4em]
        {\scriptsize\color{darkergrey}RedPajama v1}
    \end{tabular} & 
    - &
    4.0 &
    4.3 &
    4.0 &
    - &
    - &
    -
\\
    \multirow{-5}{*}{\rot{\textbf{\hspace{4em}\scriptsize{REFERENCE}}}} &
    \sans{ArXiv} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}from}
        \\[-.4em]
        {\scriptsize\color{darkergrey}pretrain}
    \end{tabular} & 
    0.5 &
    4.9 &
    5.2 &
    4.8 &
    - &
    - &
    -
\\
    \rowcolor{ai2offwhite}&
    \sans{Algebraic Stack} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}from}
        \\[-.4em]
        {\scriptsize\color{darkergrey}pretrain}
    \end{tabular} & 
    0.3 &
    2.8 &
    3.0 &
    2.7 &
    - &
    - &
    -
\\
    \rowcolor{ai2offwhite}&
    \sans{OpenWebMath} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}from}
        \\[-.4em]
        {\scriptsize\color{darkergrey}pretrain}
    \end{tabular} & 
    0.3 &
    2.9 &
    3.1 &
    2.8 &
    5.2 &
    - &
    4.8
\\
    \rowcolor{ai2offwhite}&
    \sans{GSM8k} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}train}
        \\[-.4em]
        {\scriptsize\color{darkergrey}split}
    \end{tabular} & 
    - &
    - &
    0.003 &
    0.003 &
    0.003 &
    - &
    0.003
\\
    \rowcolor{ai2offwhite}&
    \sans{Mathpile} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}commercial subset}
        \\[-.4em]
        {\scriptsize\color{darkergrey}train split}
    \end{tabular} & 
    - &
    - &
    - &
    - &
    2.1 &
    - &
    1.9
\\
    \rowcolor{ai2offwhite}
    \multirow{-5}{*}{\rot{\textbf{\hspace{2.3em}\scriptsize{MATH}}}} &
    \sans{AutoMathText} &
    \begin{tabular}{@{}l@{}}
        {\scriptsize\color{darkergrey}unfiltered}
    \end{tabular} & 
    - &
    - &
    - &
    - &
    18.5 &
    - &
    17.2
\\[.2em]
\bottomrule
\end{tabular}
\end{footnotesize}
\end{center}
\caption{
    A summary of high-quality sources we evaluate for mid-training. 
    We experiment with mixing these sources in 6 mixes, each consisting of 50 billion tokens. 
    Percentages on the table indicate the fraction of each 50B mix that is comprised by data from the respective source. 
    \MeBaseline is sampled (with repetition) from the pretraining stage. 
}
\label{table:hq_mixes}
\end{table}





==> tables/midtrain_results.tex <==
\begin{table}[h]
\centering
\begin{small}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{lcccc}
\toprule
\textbf{Mid-training mix} & \textbf{OLMES} \sans{(MCF)} & \textbf{OLMES-Gen} & \textbf{MMLU} \sans{(MCF)} & \textbf{GSM*} \\
\midrule
\rowcolor{ai2offwhite}\textit{n/a (pretrain checkpoint)} & 69.6 & 63.2 & 59.8 & 28.5 \\
\MeBaseline & 74.0 & 64.5 & 61.8 & 27.0 \\
\rowcolor{ai2offwhite}\MeDclmSeven & 73.5 & 64.1 & 61.9 & 24.5 \\
\MeFinewebThree & 73.5 & 63.0 & 62.4 & 30.5 \\
\rowcolor{ai2offwhite}\MeFinewebTwo & 75.2 & 63.8 & 63.1 & 28.5 \\
\MeFinewebTwoIns & 74.2 & 64.1 & 63.0 & 46.0 \\
\rowcolor{ai2offwhite}\MeFinewebTwoMath & {\bf75.7} & 69.7 & 62.3 & {\bf52.0} \\
\MeFinewebTwoMathIns & {\bf75.7} & {\bf70.2} & {\bf63.1} & 46.5 \\[.2em]
\bottomrule
\end{tabular}
\end{small}
\caption{
Comparison of mid-training mixes introduced in Table~\ref{table:hq_mixes}. 
Each row corresponds to a 50 billion token training run following learning rate schedule described in Section~\S\ref{sec:learning_rate_deep_dive} (except first row).
Weights are initialized from a \olmotoo checkpoint pretrained for 4T tokens. 
We compare each run on a mix of OLMES core tasks (multiple choice format; see Table~\ref{tab:evals_overview}), OLMES generative tasks (Table~\ref{tab:evals_overview}), and MMLU (multiple choice format; \citealp{hendryckstest2021}).
Results on the {\bf{final mid-training mix}}  are in Table~\ref{tab:evals-pre-post-anneal}.
}
\label{table:hq_mixes_results}
\end{table}


==> tables/sft-hypers.tex <==



\begin{figure}[h]
\centering
\begin{minipage}{0.45\textwidth}
\centering
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{cccc}
\toprule
Epochs & L.R. & Loss & Avg. Perf. \\
\midrule
2 & 1e-5 & sum & \bf{49.97} \\
3 & 4e-6 & sum & 49.76 \\
2 & 1e-5 & sum & 49.74 \\
2 & 1e-5 & sum & 49.59 \\
3 & 4e-6 & mean & 48.25 \\
2 & 2e-6 & mean & 48.18 \\
\bottomrule
\end{tabular}
\vspace{3pt}
\captionof{table}{Hyperparameter configurations tried for the 7B SFT checkpoint, all on the same dataset used in the final model. SFT models are trained with an effective batch size of 128, a linear learning rate schedule and a warmup up ratio of 0.3.}
\label{tab:sft_hypers}
\end{minipage}
\hfill
\begin{minipage}{0.45\textwidth}
\centering
\includegraphics[width=0.8\textwidth]{figures/dpo_hypers.png}
\captionof{figure}{The average score for DPO checkpoints trained on a development SFT checkpoint on different learning rates. Avg does not include Safety.}
\label{fig:dpo_lrs_plot}
\end{minipage}
\end{figure}


==> tables/soupes.tex <==
\begin{table}[h!]
\renewcommand{\arraystretch}{.8}
\begin{center}
\begin{small}
\begin{tabular}{r@{\hskip 6pt}lcccc}
\toprule
    \multicolumn{2}{c}{\textbf{Mid-training mix}} & 
    \textbf{OLMES} \sans{(MCF)} & 
    \textbf{OLMES-Gen} & 
    \textbf{MMLU} \sans{(MCF)} & 
    \textbf{GSM*} 
\\
\midrule
    \rowcolor{ai2offwhite}
    &
    best single &
    75.6 &
    68.5 &
    61.2 &
    71.0 
\\
    \rowcolor{ai2offwhite}
    \multirow{-2}{*}{A} &
    3 x soup &
    77.0 &
    69.4 &
    62.0 &
    74.0 
\\
    &
    best single &
    75.3 &
    69.9 &
    61.5 &
    73.0 
\\
    \multirow{-2}{*}{B}&
    3 x soup &
    77.3 &
    70.1 &
    62.7 &
    77.0 
\\
    \rowcolor{ai2offwhite}
    &
    best single &
    76.3 &
    70.9 &
    62.8 &
    66.0 
\\
    \rowcolor{ai2offwhite}
    \multirow{-2}{*}{C} &
    3 x soup &
    76.8 &
    71.3 &
    63.5 &
    66.0 
\\[.3em]
    &
    best single &
    77.5 &
    71.2 &
    63.4 &
    59.5
\\
    \multirow{-2}{*}{D} &
    3 x soup &
    77.8 &
    71.7 &
    63.5 &
    60.0
\\
    \rowcolor{ai2offwhite}
    &
    best single &
    73.4 &
    63.1 &
    62.2 &
    60.5
\\
    \rowcolor{ai2offwhite}
    \multirow{-2}{*}{E} &
    3 x soup &
    75.3 &
    64.2 &
    63.1 &
    43.0
\\
    &
    best single &
    77.1 &
    69.9 &
    63.7 &
    73.5
\\
    \multirow{-2}{*}{F} &
    3 x soup &
    77.9 &
    70.4 &
    63.7 &
    74.5 
\\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\caption{
Comparison of six mid-training mixes between best single checkpoint and the average of three checkpoints (\textit{soup}) trained on different data permutations. 
We run all experiments starting from 7B pretrained checkpoint; we run mid-training stage for 50B tokens. 
Souping consistently equals or outperform the single best checkpoint trained on the same mix.
}
\label{tab:soupes}
\end{table}


==> tables/stage1_vs_stage2.tex <==
\begin{table}[ht]
\setlength\tabcolsep{3pt}
\begin{center}
\begin{small}
\begin{tabular}{lc|cccccc|cccc}

\toprule
    \multicolumn{2}{l}{} &
    \multicolumn{6}{c}{\textbf{\texttt{Dev Benchmarks}}} & 
    \multicolumn{4}{c}{\textbf{\texttt{Held-out Evals}}} 
\\
    {\textbf{\fontsize{8}{8}\selectfont{Checkpoint}}} &
    {\textbf{\fontsize{8}{8}\selectfont~Avg}} &
    {\textbf{\fontsize{8}{8}\selectfont~MMLU}} & 
    {$\textbf{\fontsize{8}{8}\selectfont~ARC}_\textbf{\fontsize{6}{6}\selectfont~C}$} & 
    {\textbf{\fontsize{8}{8}\selectfont~HSwag}} & 
    {\textbf{\fontsize{8}{8}\selectfont~WinoG}} & 
    {\textbf{\fontsize{8}{8}\selectfont~NQ}} & 
    {\textbf{\fontsize{8}{8}\selectfont~DROP}} & 
    {\textbf{\fontsize{8}{8}\selectfont~AGIEval}} & 
    {\textbf{\fontsize{8}{8}\selectfont~GSM8K}} & 
    {$\textbf{\fontsize{8}{8}\selectfont~MMLU}_\textbf{\fontsize{6}{6}\selectfont~PRO}$} &
    {\textbf{\fontsize{8}{8}\selectfont~TQA}}
\\
\midrule
\rowcolor{midgrey}\multicolumn{12}{c}{\textbf{\olmotoo 1B}} \\
\rowcolor{lightgrey}{{Pretraining}} & 31.9 & 26.9 & 26.1 & 67.5 & 67.8 & 16.1 & 25.1 & 24.5 & 3.3 & 11.1 & 50.1 \\
\rowcolor{lightgrey}{{Pretraining \& mid-training}\hspace{.5em}} & 43.7 & 44.3 & 51.3 & 69.5 & 66.5 & 20.8 & 34.0 & 36.3 & 43.8 & 16.1 & 54.7 \\%[.8em]
\rowcolor{midgrey}\multicolumn{12}{c}{\textbf{\olmotoo 7B}} \\
\rowcolor{lightgrey}{{Pretraining}} & 53.0 & 59.8 & 72.6 & 81.3 & 75.8 & 29.0 & 40.7 & 44.6 & 24.1 & 27.4 & 74.6 \\
\rowcolor{lightgrey}{{Pretraining \& mid-training}\hspace{.5em}} & 62.9 & 63.7 & 79.8 & 83.8 & 77.2 & 36.9 & 60.8 & 50.4 & 67.5 & 31.0 & 78.0 \\%[.8em]
\rowcolor{ai2midwhite}\multicolumn{12}{c}{\textbf{\olmotoo 13B}} \\
\rowcolor{ai2offwhite}{{Pretraining}} & 58.9 & 63.4 & 80.2 & 84.8 & 79.4 & 34.6 & 49.6 & 48.2 & 37.3 & 31.2 & 80.3 \\
\rowcolor{ai2offwhite}{{Pretraining \& mid-training}\hspace{.5em}} & 68.3 & 67.5 & 83.5 & 86.4 & 81.5 & 46.7 & 70.7 & 54.2 & 75.1 & 35.1 & 81.9 \\
\rowcolor{ai2midpink}\multicolumn{12}{c}{\textbf{\olmotoo 32B}} \\
\rowcolor{ai2lightpink}{{Pretraining}} & 66.3 & 72.9 & 88.7 & 84.2 & 82.4 & 40.6 & 57.2 & 56.8 & 56.2 & 38.5 & 85.4 \\
\rowcolor{ai2lightpink}{{Pretraining \& mid-training}\hspace{.5em}} & 73.3 & 74.9 & 90.4 & 89.7 & 83.0 & 50.2 & 74.3 & 61.0 & 78.8 & 43.3 & 88.0 \\
\bottomrule
\end{tabular}
\end{small}
\vspace{2mm}
\caption{
Evaluations comparing \olmotoo 1B, 7B, 13B and 32B at the end of pretraining and mid-training stages (setup mirrors Table~\ref{tab:evals_overview}). 
Pretrain checkpoints have been trained on 4 trillion (1B, 7B), 5 trillion (13B) and 7 trillion (32B) tokens respectively. 
For 7B, we obtain the final mid-train checkpoints by averaging three training runs on 50B \textsc{Dolmino} tokens;
for 13B and 32B, we use three runs on 100B tokens and one run on 300B tokens.
For 1B, the final checkpoint is the result of training on 50B \textsc{Dolmino} tokens \textit{without} averaging.}
\label{tab:evals-pre-post-anneal}
\end{center}
\end{table}



==> tables/stage_1_data.tex <==

\begin{table}[h]
\centering
\small
\renewcommand{\arraystretch}{1}
\begin{tabular}{l l r r r r}
\toprule
\textbf{Source} & 
\textbf{Type} & 
\textbf{Tokens} & 
\textbf{Words} & 
\textbf{Bytes} & 
\textbf{Docs} \\
\midrule
\rowcolor{midgrey}\multicolumn{6}{c}{\textbf{\textit{Pretraining \ding{70} OLMo 2 1124 Mix}}} \\
\rowcolor{lightgrey}DCLM-Baseline & Web pages & 3.71T & 3.32T & 21.32T & 2.95B \\
    \rowcolor{lightgrey}    
    \begin{tabular}{@{}l@{}}
        \rowcolor{lightgrey}
        {StarCoder} 
        \\[-.6em]
        {
            \hspace{0.8em}
            \scriptsize
            \color{neutralFive}
            filtered version
        }
        \\[-.6em]
        {
            \hspace{0.8em}
            \scriptsize
            \color{neutralFive}
            from OLMoE Mix
        }
    \end{tabular} &
    Code & 
    83.0B & 
    70.0B & 
    459B & 
    78.7M 
\\    
    \rowcolor{lightgrey}    
    \begin{tabular}{@{}l@{}}
        \rowcolor{lightgrey}
        {peS2o} 
        \\[-.6em]
        {
            \hspace{0.8em}
            \scriptsize
            \color{neutralFive}
            from Dolma 1.7
        }
    \end{tabular} & 
    Academic papers & 
    58.6B & 
    51.1B & 
    413B & 
    38.8M 
\\
\rowcolor{lightgrey}arXiv & STEM papers & 20.8B & 19.3B & 77.2B & 3.95M \\
\rowcolor{lightgrey} OpenWebMath & Math web pages & 12.2B & 11.1B & 47.2B & 2.89M \\
\rowcolor{lightgrey}Algebraic Stack & Math proofs code & 11.8B & 10.8B & 44.0B & 2.83M \\
    \rowcolor{lightgrey}
    \begin{tabular}{@{}l@{}}
        \rowcolor{lightgrey}
        {Wikipedia \& Wikibooks} 
        \\[-.6em]
        {
            \hspace{0.8em}
            \scriptsize
            \color{neutralFive}
            from Dolma 1.7
        }
    \end{tabular} &
    Encyclopedic & 
    3.7B & 
    3.16B & 
    16.2B & 
    6.17M 
\\
\rowcolor{lightgrey}\textbf{Total} & & \textbf{3.90T} & \textbf{3.48T} & \textbf{22.38T} & \textbf{3.08B} \\
\bottomrule
\end{tabular}
\caption{
\textbf{Composition of the pretraining data for \olmotoo{}}. The \textsc{OLMo 2 1124 Mix} is composed of
StarCoder~\citep{li2023starcoder,kocetkov2022stack3tbpermissively}, peS2o~\citep{peS2o}, web text from DCLM~\citep{dclm} and Wiki come from Dolma 1.7~\citep{soldaini2024dolma}. arXiv comes from Red-Pajama~\citep{together2023redpajama},  while OpenWebMath~\citep{paster2023openwebmath} and Algebraic Stack come from ProofPile II~\citep{azerbayev2023llemma}.
}
\label{table:data-stage-1}
\end{table}


==> tables/stage_2_data.tex <==

\begin{table}[h]
\centering
\small
\renewcommand{\arraystretch}{1}
\begin{tabular}{l l r r r r}
\toprule
\textbf{Source} & 
\textbf{Type} & 
\textbf{Tokens} & 
\textbf{Words} & 
\textbf{Bytes} & 
\textbf{Docs} \\
\midrule
    \rowcolor{ai2midwhite}
    \multicolumn{6}{c}{\textbf{\textit{Mid-Training \ding{70} Dolmino High Quality Subset}}} 
\\
    \rowcolor{ai2offwhite}
    \begin{tabular}{@{}l@{}}
        \rowcolor{ai2offwhite}
        {DCLM-Baseline} 
        \\[-.6em]
        {
            \hspace{0.8em}
            \scriptsize
            \color{neutralFive}
            FastText top 7\%
        }
        \\[-.6em]
        {
            \hspace{0.8em}
            \scriptsize
            \color{neutralFive}
            $\text{FineWeb}\geqslant2$
        }
    \end{tabular} & 
    High quality web & 
    752B &  
    670B & 
    4.56T & 
    606M 
\\
    \rowcolor{ai2offwhite}
    \begin{tabular}{@{}l@{}}
        \rowcolor{ai2offwhite}
        {FLAN} 
        \\[-.6em]
        {
            \hspace{0.8em}
            \scriptsize
            \color{neutralFive}
            from Dolma 1.7
        }
        \\[-.6em]
        {
            \hspace{0.8em}
            \scriptsize
            \color{neutralFive}
            decontaminated
        }
    \end{tabular} & 
    Instruction data & 
    17.0B & 
    14.4B & 
    98.2B & 
    57.3M 
\\
    \rowcolor{ai2offwhite}
    \begin{tabular}{@{}l@{}}
        \rowcolor{ai2offwhite}
        {peS2o} 
        \\[-.6em]
        {
            \hspace{0.8em}
            \scriptsize
            \color{neutralFive}
            from Dolma 1.7
        }
    \end{tabular} & 
    Academic papers & 
    58.6B & 
    51.1B & 
    413B & 
    38.8M 
\\
    \rowcolor{ai2offwhite}
    \begin{tabular}{@{}l@{}}
        \rowcolor{ai2offwhite}
        {Wikipedia \& Wikibooks} 
        \\[-.6em]
        {
            \hspace{0.8em}
            \scriptsize
            \color{neutralFive}
            from Dolma 1.7
        }
    \end{tabular} &
    Encyclopedic & 
    3.7B & 
    3.16B & 
    16.2B & 
    6.17M 
\\
    \rowcolor{ai2offwhite}
    \begin{tabular}{@{}l@{}}
        \rowcolor{ai2offwhite}
        {Stack Exchange} 
        \\[-.6em]
        {
            \hspace{0.8em}
            \scriptsize
            \color{neutralFive}
            09/30/2024 dump
        }
        \\[-.6em]
        {
            \hspace{0.8em}
            \scriptsize
            \color{neutralFive}
            curated Q\&A data
        }
    \end{tabular} &
    Q\&A & 
    1.26B & 
    1.14B & 
    7.72B & 
    2.48M 
\\
    \rowcolor{ai2offwhite}
    \textbf{High quality total} & 
    & 
    \textbf{832.6B} & 
    \textbf{739.8B} & 
    \textbf{5.09T} & 
    \textbf{710.8M} 
\\
    \rowcolor{ai2midpink}
    \multicolumn{6}{c}{
        \textbf{
            \textit{
                Mid-training \ding{70} Dolmino Math Mix
            }
        }
    } 
\\
    \rowcolor{ai2lightpink}
    TuluMath & 
    Synthetic math & 
    230M & 
    222M & 
    1.03B & 
    220K 
\\
    \rowcolor{ai2lightpink}
    Dolmino SynthMath & 
    Synthetic math & 
    28.7M & 
    35.1M & 
    163M & 
    725K 
\\
    \rowcolor{ai2lightpink}
    TinyGSM-MIND & 
    Synthetic math & 
    6.48B & 
    5.68B & 
    25.52B & 
    17M 
\\
    \rowcolor{ai2lightpink}
    \begin{tabular}{@{}l@{}}
        \rowcolor{ai2lightpink}
        {MathCoder2} 
        \\[-.4em]
        {Synth Books} 
        \\[-.6em]
        {
            \hspace{0.8em}
            \scriptsize
            \color{neutralFive}
            Ajibawa-2023
        }
        \\[-.6em]
        {
            \hspace{0.8em}
            \scriptsize
            \color{neutralFive}
            M-A-P Matrix
        }
    \end{tabular} &
    Synthetic Math & 
    3.87B & 
    3.71B & 
    18.4B & 
    2.83M 
\\
    \rowcolor{ai2lightpink}
    \begin{tabular}{@{}l@{}}
        \rowcolor{ai2lightpink}
        {Metamath} 
        \\[-.6em]
        {
            \hspace{0.8em}
            \scriptsize
            \color{neutralFive}
            OWM-filtered
        }
    \end{tabular} &
    Math & 
    84.2M & 
    76.6M & 
    741M & 
    383K 
\\
    \rowcolor{ai2lightpink}
    \begin{tabular}{@{}l@{}}
        \rowcolor{ai2lightpink}
        {CodeSearchNet} 
        \\[-.6em]
        {
            \hspace{0.8em}
            \scriptsize
            \color{neutralFive}
            OWM-filtered
        }
    \end{tabular} &
    Code & 
    1.78M & 
    1.41M & 
    29.8M & 
    7.27K 
\\
    \rowcolor{ai2lightpink}
    \begin{tabular}{@{}l@{}}
        \rowcolor{ai2lightpink}
        {GSM8K} 
        \\[-.6em]
        {
            \hspace{0.8em}
            \scriptsize
            \color{neutralFive}
            Train split
        }
    \end{tabular} &
    Math & 
    2.74M & 
    3.00M & 
    25.3M & 
    17.6K 
\\
    \rowcolor{ai2lightpink}
    \textbf{Math total} & 
    & 
    \textbf{10.7B} & 
    \textbf{9.73B} & 
    \textbf{45.9B} & 
    \textbf{21.37M} 
\\
\bottomrule
\end{tabular}
\caption{
\textbf{Composition of the mid-training data (Dolmino)}.  
From this set, we create samples of 50B, 100B and 300B tokens to mid-train \olmotoo on. 
See Section~\S\ref{sec:diveAnnealing} for details regarding individual source details, and Table \ref{tab:dolmino-composition-pretty} for the specific composition of each annealing mixture.
}
\label{table:stage-2-data}
\end{table}

